Question Rewriting for Conversational Question Answering

Conversational question answering (QA) requires the ability to correctly interpret a question in the context of previous conversation turns. We address the conversational QA task by decomposing it into question rewriting and question answering subtasks. The question rewriting (QR) subtask is specifically designed to reformulate ambiguous questions, which depend on the conversational context, into unambiguous questions that can be correctly interpreted outside of the conversational context. We introduce a conversational QA architecture that sets the new state of the art on the TREC CAsT 2019 passage retrieval dataset. Moreover, we show that the same QR model improves QA performance on the QuAC dataset with respect to answer span extraction, which is the next step in QA after passage retrieval. Our evaluation results indicate that the QR model we proposed achieves near human-level performance on both datasets and the gap in performance on the end-to-end conversational QA task is attributed mostly to the errors in QA.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> scrap.tex <==
% Moreover, our conversational QA architecture based on question rewriting sets the new state of the art on the TREC CAsT 2019 dataset with a 28\% improvement in MAP and 21\% in NDCG@3.
%Moreover, we show that the same question rewriting model can be adopted to extend answer extraction to a conversational setting as well.
% report performance on the CANARD test split of QuAC, an extractive conversational QA dataset, which is achieved with the same QR model used for TREC CAsT. 
% more conretely what are the insights over QR/QA interplay
% Our detailed analysis of the evaluation results provide insights into the 
%contribution
% We also report on the correlation between intrinsic evaluation measures of the text generation quality for question rewriting and performance on the end-to-end QA tasks.
% and show the lack of robustness in reading comprehension models.
% , and demonstrates the strengths and weaknesses of the retrieval and extractive QA architectures, that should be reflected in their integration.
% Our detailed analysis of the results, which uses question rewriting as a mechanism for evaluation of the impact of variance in question formulation on the QA performance, casts light on the weaknesses in both retrieval and extractive QA architectures that should be reflected in their integration.
% Of the four question rewriting techniques we assessed, the Sequence-to-Sequence model, as used in the original CANARD paper, performed the worst.
% However, using this model as a question rewriter is still roughly comparable to training a typical conversational question answering model from scratch, designed specifically to model previous dialogue turns as well.
% The other QR models all performed better, with the Action-Generator reaching the best F1 of $58.16$.

% As shown in Table ~\ref{table:trec}, using the IDF keywords from $k$ previous turns to augment the original implicit question actually forms a strong baseline, beating the much more complicated S2S and Co-Ref with BERT models on all three evaluation metrics. However, both the PG and AG models beat the baselines by a large margin. Using the manual human rewrites with BERT sets the upper bound of the query rewriting approach and is better than the best model rewriter.

% We further analyse the type of errors based on the samples obtained from the break-down subgroups (Table~\ref{table:trec_breakdown}) and the outliers identified during the correlation analysis.
% All errors stem from two major root causes of deviation: sensitivity of the QA component and completeness of the question rewrite, both of which we further describe and exemplify below.


% task
% Given a conversation context $C$ (previous conversational turns in our case) and a potentially implicit question $Q$, which may not be correctly interpretable outside of the conversation context $C$, the task of a question rewriting (QR) model is to generate an explicit question $Q'$ which is equivalent to $Q$ under conversation context $C$ and has the same correct answer $A$.
% % model architecture
% Our approach to question rewriting builds upon a Transformer decoder architecture (GPT model)~\cite{radford2019language}.
% \todo{@SV briefly describe the model and fix the figure accordingly}
% % that embeds the conversation and then projects its embedding into the vocabulary distributions restricted to the tokens present either in the implicit question $Q$ or the conversation context $C$~\cite{qrecc2020} (see Figure~\ref{fig:qr} for the model overview).
% % input
% We concatenate the question and previous conversation turns with a separation token in between and use this sequence as a model input.
% In our experiments, we used 5 previous conversation turns as input to the QR model.


% question and context vocabulary distributions

% Input Embeddings ($E_I$) for each token $w_t$ is the sum of its token embedding ($E_W$) and the position embedding ($E_P$):
% \begin{equation}
%     E_I =  E_W + E_P
% \end{equation}
% \todo{different from the original formula}

% The input embeddings are encoded using Transformer producing a sequence of hidden states $h_t$:
% \begin{equation}
%     h_t = \text{Transformer}(E_I(w_t), h_{t-1})
% \end{equation}

% The hidden states are fed through the question and context Language Modeling (LM) heads to obtain question ($Q'_Q$) and context ($Q'_C$) vocabulary distributions:
% \begin{equation}
%     Q'_Q = \text{softmax}(w_{q}h_t+b_{q})
% \end{equation}
% \begin{equation}
%     Q'_C = \text{softmax}(w_{c}h_t+b_{c})
% \end{equation}

% % question and context vocabulary distribution weights
% Attention distribution for the question Q' is given by multi-head attention on hidden states:
% \begin{equation}
%     a_{Q'} = \text{MultiHead}_{Q'}(h_t)
% \end{equation}

% The encoder hidden states $h_t$ are weighted with the attention distribution $a_{Q'}$ and summed to produce a context vector $h^*_{Q'}$ for the question $Q'$:
% \begin{equation}
%     h^*_{Q'} = \sum{a_{Q'} \cdot h_t}
% \end{equation}

% These results have direct implications on the type of datasets and the range of tasks required to design a robust system for conversational QA.

% optimised recall precision
% Our experiments show that \todo{@SV report main lessons learned from the evaluation results also in relation to other experiments on retrieval+extractive QA architectures HotpotQA and ELI5}
% to retrieve relevant documents and then use them to directly extract or generate an appropriate answer

% future work: integration

% This setup allows us to inspect the flaws of the individual QA components and predict the effect from combining them into a single architecture.

% The preactivation for probability weight of question vocabulary distribution is computed as:
% \begin{equation}
%     z_Q = w_{h^*_Q}h^*_{Q'} + w_{s_Q}s + w_{x_Q}x + b_{Q}
% \end{equation}
% where $s$, $x$ denote decoder state and decoder input respectively. $w_{h^*_Q}$, $w_{s_Q}$, $w_{x_Q}$, and $b_{Q}$ are learnable parameters.

% Similarly, the preactivation for probability weight of context vocabulary distribution is computed as:
% \begin{equation}
%     z_C = w_{h^*_C}h^*_{C} + w_{s_C}s + w_{x_C}x + b_{C}
% \end{equation}
% where $h^*_{C}$ denotes context vector of conversation context. $w_{h^*_C}$, $w_{s_C}$, $w_{x_C}$, and $b_{C}$ are learnable parameters.

% The probability weights for question and vocabulary distributions are given by:
% \begin{equation}
%     w_Q, w_C = \text{softmax}(z_Q, z_C)
% \end{equation}

% Thereby, the output of the model, which is an explicit question $Q'$, is produced by recursively sampling tokens from the distribution $P(x \in Q_i \cup C_i)$, which is to be learned during the training procedure.

%  equipped with two pointer-heads. Every output token is produced by a weighted sum of two vocabulary distributions over the tokens from the original implicit question $Q'_Q$ and the previous conversation turns $Q'_C$.

% output
% Every output token is produced by a weighted sum of two vocabulary distributions over the tokens from the original implicit question $Q'_Q$ and the previous conversation turns $Q'_C$:
% \begin{equation}
%     Q' =  w_Q \cdot Q'_Q + w_C \cdot Q'_C
% \end{equation}

% As shown in Table ~\ref{table:quac}, we compare our question rewriting and pre-trained MultiQA model against alternative methods, as well as the human rewritten upper bound. The CANARD + $k$-DT refers to CANARD training set where $k$ prior dialogue turns are fed as additional inputs to the extractive QA model. We also compare the results using different question rewriting techniques at evaluation time, including the Sequence-to-Sequence (S2S), Co-Reference (Co-Ref), Pointer-Generator (PG), and Action-Generator (AG) models, described in Section~\ref{sec:qr_models}.
% The Exact Match (EM) and F1 scores show (a) that our query rewriting method at evaluation time is competitive, and even exceeds, alternative methods without custom modifications to accommodate prior conversational context, and (b) that a query re-writer matching human performance would provide the best results of all (the Human-CANARD upper bound).
% In Figure~\ref{fig:canard-breakdown} we analyze how a QA model trained on full-context questions performs on context-unaware "Original", Action-Generator rewritten, and "Human" rewritten questions. This figure is akin to Table~\ref{table:quac_breakdown} but depicts the number of examples per category over the entire scale of F1 thresholds (the x-axis). This breakdown illustrates how question rewrites affect the QA model's ability to select the correct answer. If we examine only the pink region of the chart (Original (1), QR (1), Human (1), where $F1\ge1.0$ (at the very right of the Figure), the height of this region represents all queries in the CANARD test set for which the QA model is always able to find an answer, where $F1\ge1.0$ (or $EM=1.0$), for any of Original, QR, or Human versions of the question. This corresponds to about 40\% of the test set. If we reduce the F1 score threshold required to say the answer is sufficient, from 1 to 0 (now the left side of the Figure) we see the proportion of the test set rises to nearly 70\%. The blue region of the chart represents examples for which no version of the query is sufficient for the QA model to get a sufficient answer, and thus question rewriting did not help. This region represents the shortcomings of the QA model, which should theoretically be able to answer any question once human rewritten.

% The regions that illustrate the weakness of the question rewriting approach are those where QA model actually prefers the original question, as with the green region (Original (1) | QR (0) | Human (0)), or where our best QR model degrades the query below original, or human versions, as with the yellow region (Original (1) | QR (0) | Human (1)). Fortunately, both these regions are relatively small, with $2.9$\% and $0.59$\% of the test set respectively, when $F1=1.0$.

% The regions that illustrate the strengths of the question rewriting approach are relatively larger. Consider examples where our rewriting improves the QA performance, as with the turquoise region (Original (0) | QR (1) | Human (1)), or where the QA model only succeeds with the Human rewritten question, as with the orange region (Original (0) | QR (0) | Human (1)). These regions constitute $4.8$\% and $4.2$\% of the test set respectively, when $F1=1.0$.


% In Table~\ref{table:quac_breakdown}, we see how the model trained on Human rewritten inputs for the CANARD set performs on a question in its different forms: original, model rewritten, and human rewritten. The column with $1$ for each of "original", "QR" and "human" indicates examples where the model achieved a strong answer when evaluated on every form of the question. The number of examples that are measured as "strong" answers are tallied according to whether they exceed a given F1 threshold: $0$, $0.5$, and $1$ in the columns respectively.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/map_thresholds}
%   \caption{For each example in the TREC CAsT test set we evaluate the system's performance on each of the three question types, "Original", Action-Generator rewritten, and "Human" rewritten, and record the respective MAP values. For a given MAP threshold we aggregate examples according to which types of queries the system achieved better (1) or worse (0) than the F1 threshold. These aggregated groups are visualized as colours, as shown by the legend Score Card.}
%     \label{fig:treccast-breakdown}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/canard-breakdown.png}
%   \caption{An illustration of how a QA model trained on full-context questions performs on context-unaware "Original", Action-Generator rewritten, and "Human" rewritten questions. For each example in the CANARD test set we evaluate the model's performance on each of the three question types, and record the respective F1 scores. For a given F1 Threshold we aggregate examples according to which types of queries the model achieved better (1) or worse (0) than the F1 threshold. These aggregated groups are visualized as colours, as shown by the legend Score Card.}
%     \label{fig:canard-breakdown}
% \end{figure}



% the evaluation metric for text generation, while incapable to cover complex semantic paraphrases, still correlates well with the standard QA metric on the end-to-end task and is, therefore, sufficiently reflects the quality of question rewriting, as an ability of the system to understand the question in the context of a conversation and formulate an adequate query for the down-stream QA components.

% extractive QA breakdown
% A breakdown of a QA model's predictions on "original", query rewritten "QR", and "human" rewritten questions. The value one (1) indicates the model exceeded the F1 threshold for a particular example, whereas (0) indicates the model did not. The number of examples are tallied according to F1 thresholds in the three rightmost columns.


% Table~\ref{table:trec_breakdown} breaks down the number of conversation turns where the top ranked answer is relevant for each implicit, QR, and human rewrite combination.
% For example, the (Original (0) | QR (1) | Human (1)) column shows the number of turns where the original implicit cannot find a relevant answer in the top hit, but the top query rewriting method (AG) and human rewrite can. 
% Overall there are 49 (28.3\%) turns where neither of the methods can find the relevant answer as the top hit, where for 55 (31.8\%) turns all three methods can find the relevant answer as the top hit.
% There are no test set turns where the implicit question can find the answer as the top hit, but query rewriting and human rewriting cannot.
% Human rewriting can also get all the turns that implicit question and query rewriting can get correct (top hit is relevant).
% However, surprisingly, there are 2 turns where query rewriting can get the relevant answer in the top hit, but implicit question or even human rewriting cannot.

% In the bottom half of Table~\ref{table:trec_breakdown}, we see that there are no turns where implicit question and human rewriting can get a turn correct but query rewriting cannot.
% There are 19 (11.0\%) turns where human rewriting can get a turn correct, but the best query rewriting model cannot, indicating the gap between the AG model and human rewriting model still.
% However, there are many more cases, 48 (27.7\%) that the best query rewriting model as well as the human rewriting model can get correct over just using implicit question than the cases that query rewriting misses, but human rewriting gets correct.
% Overall, we see that query rewriting can get all turns where the implicit question can get correct, and catch a significant number of turns correct where the implicit question misses.
% Human rewriting is still the best, but surprisingly query rewriting can actually get two turns correct that human rewriting misses.


% Furthermore, it is clear from this table that 

% QR component failed to match human performance in 19 cases (11\% of all samples in the TREC CAsT test set).
% This analysis suggests that the main bottleneck remaining in this task of conversational QA is the performance of the retrieval component.
% The QR component we proposed does provide an important value by bringing in 50 (48 + 2) rewrites (29\% of the test set samples) that allow to accurately interpret these questions with respect to the conversation context and are instrumental in retrieving the correct answers from the passage collection.

% retrieval QA breakdown
% The number in parenthesis indicates the number of relevant turns where the implicit question is the same as human rewrite. Out of the 14 questions where implicit question and human rewrites are the same and both got a bad top hit, 12 questions come from the first turns of their respective conversations.
% The first number in parenthesis corrects this estimate for question rewriting by removing the number of all first questions per conversation because they are copied without rewriting by default. The second number is parenthesis indicates the number of questions that are not first questions in the conversations 

